Duration-Differentiated Services in Electricity

The integration of renewable sources poses challenges at the operational and economic levels of the power grid. In terms of keeping the balance between supply and demand, the usual scheme of supply following load may not be appropriate for large penetration levels of uncertain and intermittent renewable supply. In this paper, we focus on an alternative scheme in which the load follows the supply, exploiting the flexibility associated with the demand side. We consider a model of flexible loads that are to be serviced by zero-marginal cost renewable power together with conventional generation if necessary. Each load demands 1 kW for a specified number of time slots within an operational period. The flexibility of a load resides in the fact that the service may be delivered over any slots within the operational period. Loads therefore require flexible energy services that are differentiated by the demanded duration. We focus on two problems associated with durations-differentiated loads. The first problem deals with the operational decisions that a supplier has to make to serve a given set of duration differentiated loads. The second problem focuses on a market implementation for duration differentiated services. We give necessary and sufficient conditions under which the available power can service the loads, and we describe an algorithm that constructs an appropriate allocation. In the event the available supply is inadequate, we characterize the minimum amount of power that must be purchased to service the loads. Next we consider a forward market where consumers can purchase duration differentiated energy services. We first characterize social welfare maximizing allocations in this forward market and then show the existence of an efficient competitive equilibrium.

==> 01intro.tex <==
\section{Introduction} \label{sec-introduction}
The worldwide interest in renewable energy such as wind and solar is driven by pressing environmental problems, energy supply security and nuclear power safety concerns. The energy production from these renewable sources is {\em variable}: uncontrollable, intermittent, uncertain. 
Variability is a challenge to deep renewable integration.

A central problem is that of economically balancing demand and supply of electricity in the 
presence of large amounts of variable generation. The current {\em supply side} approach 
is to absorb the  variability in operating reserves.
Here, renewables are treated as negative demand, so the variability appears as uncertainty in net load which is compensated by scheduling  fast-acting reserve generation.  This strategy of {\em tailoring supply to meet demand} works
at today’s modest penetration levels. But it will not scale. Recent studies in California, e.g., \cite{CAISO},  project that the load-following capacity requirements will need to increase from 2.3 GW to 4.4 GW. These large increases in reserves will significantly raise electricity cost, and diminish the net carbon benefit from renewables as argued in several papers in the literature (\cite{kirschen2010,negwankowshamey12}).

There is an emerging consensus that demand side resources must play a key role in supplying zero-emissions regulation services that are necessary for deep renewable integration  (e.g., \cite{cal09K, galus2010, papaoren2010, matdyscal12K, anand2012}). These include thermostatically controlled loads (TCLs), electric vehicles (EVs), and smart appliances.  Some of these loads are deferrable: they can be shifted over time.  For example, charging of electrical vehicles (EVs) may be postponed to some degree.    Other loads such as HVAC units can be modulated within limits.  
The core idea of {\em demand side approaches} to renewable integration is to exploit load flexibility to 
track variability in supply, i.e., to tailor demand to match supply.  For this a cluster manager or aggregator 
offers a control and business interface between the loads and the system operator (SO). 

%%%NEW
The demand side approach has led to two streams of work: (a) indirect load control (ILC) where flexible loads respond, in real-time, to price proxy signals, and (b) direct load control (DLC) where flexible loads cede physical control of devices to operators who determine appropriate actions. The advantage of DLC is that with greater control authority the cluster manager can more reliably control the aggregate load.  
However, DLC requires a more extensive control and communication infrastructure and the manager must provide economic incentives to recruit a sufficient consumer base. The advantage of ILC is that the consumer retains authority over her electricity consumption.  

%For DLC to be effective, the electric service that is
%sold must be  designed to take advantage of the flexibility in the loads, which will need control schemes to 
%implement the commodity transactions.


Both ILC and DLC require appropriate economic incentives for the consumers.  In ILC, the real-time price signals provides the required incentives. However, the quantification of those prices, the feasibility of consumer response and the impact on the system and market operations in terms of price volatility and instabilities is a matter of concern, as recent literature suggest (\cite{RoozbehaniCDC2010,LBNL-RTPReport,wannegkowshameysha11b}).  

DLC also requires the creation of economic signals, but unlike real-time pricing schemes DLC can  use forward markets. For DLC to be effective, it is necessary to offer consumers who present greater demand flexibility a larger discount. The discounted pricing can be arranged through flexibility-differentiated electricity markets. Here, electricity is regarded as a set of differentiated services as opposed to a homogeneous 
commodity.  Consumers can purchase an appropriate bundle of services that best meets their electricity needs.
From the producer's perspective, providing differentiated services may better accommodate supply variability. 
This paper is concerned with electric power services differentiated by the duration $h$ for which power is supplied. 
We explore balancing supply and demand for such services through forward markets.
There is a growing body of work \cite{tanvar93, pravin2011,negmey12, bitar2013} on differentiated electricity services. 

%The demand side approach has led to two streams of work: (a) indirect load control (ILC) where flexible loads respond, in real-time, to price proxy signals to persuade consumers to change consumption appropriately, and (b) direct load control (DLC) where flexible loads cede physical control of devices to operators who determine appropriate actions. The advantage of DLC is that with greater control authority the cluster manager can more reliably control the aggregate load.  
%However, DLC requires a more extensive control and communication infrastructure and the manager must provide economic incentives to recruit a sufficient consumer base.
%The advantage of ILC is that the consumer retains authority over her electricity consumption.  
%For ILC to be effective, the electric service that is
%sold must be  designed to take advantage of the flexibility in the loads, which will need control schemes to 
%implement the commodity transactions.
%
%In indirect load control, flexible loads can be regarded as accepting quality-differentiated electric power services.
%Consumers offering greater flexibility receive discounted electricity prices through a market constructed to deliver these services from producers with variable generation. Such markets require a radical shift in how we think of electricity – not as an undifferentiated good, but rather as a set of differentiated services from which individual consumers can specify a 
%quality-of-service that best meets their electricity needs. From the producer perspective, 
%selling these differentiated services is better suited to accommodate supply variability. This paper is concerned 
%with electric power services
%over a service horizon differentiated by the duration $h$ for which power is supplied. We explore balancing supply and demand
%for such services through forward markets.

\subsection{Prior Work} \label{sec-prior}

\subsection*{Supply side approaches} 

Here, variable supply from renewable sources is regarded as negative demand.
The objective is to arrange for reserve power generation to compensate for fluctuations in net demand.  
The problem is formulated from the viewpoint of the system operator (SO)
who must purchase reserve generation capacity and energy to meet the random demand while 
minimizing the risk of mismatch and the cost of reserves. 
Reserve generation can be purchased in forward markets with different time horizons (day-ahead, hour-ahead, 5 minutes-ahead).
With shorter time horizons, the uncertainty in the forecast net demand is reduced but the cost of reserves increases.  
The SO's  optimal decision can be formulated as a stochastic control problem known as risk-limiting dispatch presented in \cite{pravin2011}.  
When SO's decisions include unit commitment  and transmission constraints, the problem 
is a mixed-integer nonlinear stochastic programming problem that is computationally challenging as discussed in \cite{galiana}. A number of papers address the
computational aspects of stochastic unit commitment (e.g., \cite{carpentier1996, nowak2000, paporeone2011}). Alternatively, \cite{berlitsun2013} present a robust optimization formulation of the unit commitment problem. If unit commitment and transmission constraints are omitted, the resulting stochastic dispatch problem has an analytical solution as shown in \cite{varaiya_rld, PMAPS2012}. 

\subsection*{Demand side approaches}

Current research in {\em direct load control}  focuses on developing and analyzing algorithms for coordinating resources (e.g., \cite{ChenLLF2011, LeeTPS2008, HsuDLC1991, MetsEVCharging2010}). For example, \cite{GanPESGM2012} develops a distributed scheduling protocol for electric vehicle charging; \cite{papaoren2010} uses approximate dynamic programming to couple wind generation with deferrable loads; and \cite{MaIFAC2011, GHGIREP2010, galus2010} suggest the use of receding horizon control approaches for resource scheduling.

Recent studies in {\em indirect load control} have developed real-time pricing algorithms \cite{IlicTPSNov2011} and
quantified operational benefits \cite{LijesenRTPElasticity}.  There has also been research focused on economic efficiency in \cite{Borenstein2005,Spees2007}, feedback stability of price signals in \cite{RoozbehaniCDC2010}, volatility of real-time markets in \cite{wannegkowshameysha11b} as well as the practical issues associated with implementing ILC programs presented in \cite{LBNL-RTPReport}. 

An early exposition of differentiated energy services is offered in \cite{OrenSmith}.
There are other approaches to such services that naturally serve to integrate variable generation sources. 
Reliability differentiated energy services where consumers accept contracts for $p$ MW of power with probability $\rho$ are developed in \cite{tanvar93}. More recently, the works of \cite{bitarlow2012, bitar2013} consider deadline differentiated contracts where consumers receive price discounts for offering larger windows for the delivery of $E$ MWh of energy. 

\subsection{Main Contributions}

%%NEW
In this paper, we consider a class of flexible loads that require a fixed power level for a specified duration within an operational period. The loads are differentiated based on the duration of service they require, we refer to them as duration-differentiated (DD) loads. We consider a stylized version of DD loads. The service interval is divided into $T$ slots, indexed $t = 1, \cdots, T$. A flexible load demands 1 kW of power for a duration of $h$ slots.  While this abstraction does not account for many important practical constraints, it serves to formulate and study the central mathematical problems in scheduling/control and markets for DD loads. The flexibility of a load resides in the fact that {\em any} $h$ of the available $T$ slots will satisfy the load. Examples of DD loads include electric vehicles that allow flexible charging over an 8 hour service interval, aluminum smelters that might operate for $h$ hours out of $24$, appliances such as washing machines that require a fixed power for any $1$ hour out of the next $8$. 
%%

%This paper considers a stylized version of flexible loads. The service interval is divided into $T$ slots, indexed $t = 1, \cdots, T$. We assume the available power $p_t$ kW in any slot $t$ is given.
%A flexible load demands 1 kW of power for a duration of $h$ slots.  While this abstraction does not account for many important practical constraints, it serves to formulate and study the central mathematical problems in scheduling/control and economics for DD loads.

%The flexibility resides in the fact that {\em any} $h$ of the available $T$ slots will satisfy the load.   
%%A load requiring power for $h_1$ slots offers more flexibility that one requiring power for $h_2 > h_1$ slots. 
%There are  $N$ loads, defined by their service durations $h = \{h_i, i=1, \cdots, N\}$.  
%%The consumers or loads can be regarded as demanding duration differentiated energy services.

%We take a demand side approach with direct load control. 
Our objective is to study the allocation of available supply to the various loads in a market context. 
%Loads are induced to participate in this market by receiving lower electricity prices in exchange for greater flexibility.
We assume that if the supplier contracts {\em ex ante} to deliver power for $h$ slots to a particular flexible load, it is obligated to do so. The supplier selects $h$ of the the available $T$ slots to supply power to the load. This scheme requires certain technology infrastructure (communication, power electronics), a treatment of which is outside the scope of this paper. The load is not informed much in advance which $h$ slots it will receive power. Thus the load must assume the burden of planning its consumption without knowing exactly when power will be available. The available power is drawn from zero-marginal  cost renewable sources as well as electricity purchases made by the supplier in the day-ahead. Because of the variability in renewable sources, the supplier may be compelled to use supplemental generation such as on-site gas turbine or buying from a real-time market to meet its obligations.

%We focus on operational and market aspects of DD loads. Firstly, we address the supplier's decision problems for serving a given set of DD loads.  We provide a complete characterization of supply adequacy, an algorithm for allocating supply to meet the loads and the optimal policies for making day-ahead and real-time power purchase decisions. On the economic side, we  study a simplified model of a forward market for DD loads where supply uncertainty is not explicitly taken into account.  For this market model, we present the centralized solution that maximizes social welfare and characterize an efficient competitive equilibrium. We also contrast this equilibrium with the outcome of a stylized real-time market.

Our first set of results are contained in Section \ref{sec:discrete}. Here, we study the decision problems faced by a supplier who has to serve a fixed set of DD loads.  The basic question we address is the following: given a forecast model of its renewable generation, what day-ahead and real time power purchases should a supplier make to ensure that all loads are served at least possible cost? To solve this problem, 
we first give a necessary and sufficient condition under which the available power $\mathbf{p}= (p_1, p_2, \ldots,p_T)$ is adequate to meet the loads. We describe a Least Laxity First (LLF) algorithm that constructs an appropriate allocation to serve the loads.   
%The flexibility in demand is used to shape the time profile of the loads to match the inflexible time profile of the available power.
In the event the available supply profile $\mathbf{p}$ does not meet the adequacy condition, we characterize the minimum cost power purchase decisions under (a) oracle information, and (b) run-time information about the supply. We use this solution to construct optimal day-ahead and real-time decisions for the supplier in Section~\ref{sec:supplier_problem}. %Finally, we treat the more general case where load $i$ must be supplied $E_i$ kW-slots of power at a maximum rate of $m_i$ kW per slot.  

Our second set of results may be found in Section \ref{sec:market}. Here, we consider a stylized {\em forward market for duration-differentiated services}, which are bundles of  $h$ 1-kW slots sold at prices $\pi(h)$, $h=1,2, \cdots$.  
Consumer $i$ select the service $h$ that maximizes her net utility $U(h) - \pi(h)$,
and the supplier bundles its supply  (both its renewable generation and any forward purchases made from the grid) into 
$n_h$ units of service for $h$ slots, so as to maximize its revenue.  We show that there is a competitive market equilibrium which maximizes social welfare.  The competitive duration-differentiated market equilibrium is then compared with a sequential real-time market, 
in which the price of power $\zeta (t)$ is the market clearing price for slot $t$.  
The comparison reveals that the real-time markets may not be efficient.
%price will be more volatile than the prices of the duration-differentiated services.  
%This may be expected since the latter incorporates a kind of {\em forward} market.  The reduced price
%volatility may make duration-differentiated services attractive to both consumers and suppliers. 
All proofs are collated in the Appendix. Concluding remarks and future research avenues are discussed in Section \ref{sec-conclusions}.



%\subsubsection*{Demand side approaches: ILC}

\subsection*{Notation}

Bold letters denote vectors. We reserve subscripts $t$ to index time and $i$ to index loads.
For a vector $\VEC a =(a_1,a_2,\ldots,a_T)$, $\VEC a^{\downarrow}$ denotes the non-increasing 
rearrangement of $\VEC a$, so, $a^{\downarrow}_t \geq a^{\downarrow}_{t+1}$ for $t=1,2,\ldots,T-1$.
For an assertion $A$, $\mathds{1}_{A}$ denotes $1$ if $A$ is true and $0$ if $A$ is false. 


%Next, we suppose consumers have (identical) utility functions $U(E,M)$, and we find the allocation that maximizes the social welfare, $\sum_n U(E_n,M_n)$.  We show that the optimum allocation can be sustained as a competitive equilibrium in which consumers can purchase commodities comprised of 1 kW of power of variable duration $h= 1, \cdots, T$, at prices $\pi(h)$.  

%In the continuum case a load  specified by a pair $(\ell, h)$ requires $\ell$ kW of power for $h$ slots.  There is a continuum of loads $(\ell(x), h(x))$, indexed by $x \in [0,1]$.  Again, we give conditions under which the available power $(p_1, \cdots, p_T)$ can meet the loads.  We consider the situation in which the  the available power is divided into packages of power differentiated by duration and amount.  We suppose that consumer $x$'s  utility function is $U(x, \ell, h)$, find the allocation that maximizes the social welfare $\int_0^1 U(x, \ell(x), h(x))dx$.   We show that there is a market equilibrium in which consumers'  purchases coincide with this allocation.

%\subsection{Organization of Paper}
%Section \S\ref{sec-two} considers the basic problem of allocating a supply profile to a set of loads, 
%when both are known in advance.  All proofs are collated in the Appendix.
%






==> 02adequacy.tex <==



\section{Problem Statement}\label{sec:PF}
We formalize the two problems investigated in this work. The first problem deals with the operational decisions that a supplier has to make to serve a given set of duration differentiated loads. The second problem focuses on a market implementation for duration differentiated services.

%\subsection{Setting}




\subsection{Serving a collection of duration differentiated loads}
We consider a discrete-time setting where time is segmented into $T$ slots, indexed by $t$.   The power available in slot $t$ is assumed to take non-negative integer values. 
There are  $N$ flexible loads, indexed by $i$. Load $i$ requires $1$ kW for {\em any}  $h_i$  of $T$ time slots.  The vector $\VEC h = (h_1,h_2,\ldots,h_N)$ is called the \emph{demand profile}.  For a demand profile $\VEC h$, we define an associated \emph{demand-duration vector} $\VEC d = (d_1,d_2,\ldots,d_T)$ where $d_t := \sum_i\mathds{1}_{\{t \leq h_i\}}$. Note that the number of consumers that need service for $t$ slots is  $d_t - d_{t+1}$ (where $d_{T+1} := 0$). Thus, there is a bijection between the demand profile and the demand-duration vector as $\VEC h$ specifies $\VEC d$ uniquely and {\em vice versa}.  

We consider the supplier's problem of serving a given collection of these  loads. The supplier owns renewable energy resources that can provide free but uncertain power. In addition, the supplier can purchase power in the day-ahead and real-time electricity markets. The renewable generation over the delivery period is denoted by the  non-negative integer-valued random vector  $\VEC R = (R_1,R_2,\ldots,R_T)$; the realizations of this vector are denoted by $\VEC r$. In the day-ahead market, the supplier has a probability mass function on this random vector given by $f(\VEC r)$. If the supplier purchases a power profile $\VEC y = (y_1,y_2,\ldots,y_T)$ in the day-ahead market, its cost is given by $c^{da}(\sum_{t=1}^T  y_t)$, where $c^{da}$ is day-ahead market price. In real-time, the random vector of renewable generation takes a realization $\VEC r$, so that the total realized supply profile is $\VEC p = \VEC r+ \VEC y$. Since, this supply may not be adequate for serving all the loads, the supplier may have to purchase additional energy at the real-time market price $c^{rt}$. We assume that over the time of actual delivery, the supplier sequentially observes the true realizations of its renewable  power in each slot and makes a real-time purchase decision $a_t$ in slot $t$ according to a \emph{decision policy} of the form
 \begin{equation}
 a_t = g_t(\VEC y, r_1,r_2,\ldots,r_t)
 \end{equation}%Since the loads are flexible, many supply profiles can service a given load profile. 
 
 For a given day-ahead purchase decision $\VEC y$ and a real-time decision rule $\VEC g = (g_1,g_2,\ldots,g_T)$, the supplier's total expected cost is given as
 \begin{equation} \label{eq:expected_cost}
  \mathcal{J}(\VEC y, \VEC g) := c^{da}\sum_{t=1}^T y_t + c^{rt}\mathds{E} \Bigg[ \sum_{t=1}^T g_t(\VEC y, R_1,R_2,\ldots,R_t)\Bigg],
 \end{equation}
 where the expectation is over the random vector $\VEC R$. The supplier's problem can be stated as follows.
 \begin{problem}
 What choice of the  day-ahead purchase decision $\VEC y$ and the real-time decision rule $\VEC g = (g_1,g_2,\ldots,g_T)$ minimizes the total expected cost given by \eqref{eq:expected_cost} while ensuring that all loads are served?
 \end{problem}
 
 
 
 
\subsection{Forward market for flexible services}
In Problem 1, the set of duration-differentiated  loads was assumed to be fixed. We would like to investigate  how this set of duration-differentiated loads results from a market interaction between consumers and suppliers. 
We consider a forward market for duration-differentiated services.   All the market transactions between the consumers and the suppliers are completed before the operational period. %Thus, the market decisions are made prior to the operational decisions required for the delivery of the products which is a characteristic of direct load control. 
The forward market has three elements:

\balphlist
\item Services: The services are differentiated by the number $h$ of time slots within $T$ slots during which 1 kW of electric power is to be delivered.  Service $h$ is sold at price $\pi(h)$.
\item Consumers: The benefit to a consumer who receives $h$ slots is  $U(h)$; all consumers have the same utility function $U$. 
\item Supplier: The supplier receives for free the power with profile $\VEC R = (R_1, \cdots, R_T)$.    The supplier cost is given by $\mathcal{J}(\VEC y, \VEC g)$ as defined by \eqref{eq:expected_cost} in the previous section.
\end{list}
%, $\VEC h = (h_1,h_2,\ldots,h_N)$ in which $h_i$ represents the duration that consumer $i$ is receiving,

In order to make the analysis tractable, we focus on idealized market structure  and supplier behavior. In particular, we assume  a competitive market setting in which all agents act as price takers. We also assume that while making their market decisions, suppliers ignore the forecast errors about their renewable supply. 
In this setting, we consider the following problem.
%\begin{enumerate}
%\item Competitive Market: Suppliers and consumers are assumed to be price takers without the possibility of impact the market prices.
%\item Certainty Equivalence: In order to make their market decision, the suppliers ignore the uncertainty in their forecast by treating their expected value of renewable power as the true realization. 
%\end{enumerate}
%The first assumption is standard in market analysis in which price are assumed to be exogenous to the players decisions. The second assumption allows to simplify the suppliers problem in the market setting. It avoids the need to consider the costs resulting from the two-stage optimization problem presenting previously. While making its forward market decisions, the supplier only takes into account to its day-ahead energy purchases. We further assume that the day-ahead energy cost is linear and is given as  $C\VEC 1^t \VEC y$ in which $C$ represents the day-ahead market price.%By assuming this, the additional power cost will be just $C\VEC 1^t \VEC y$ in which $C$ represents the day-ahead market price.  
\begin{problem}
 Is there a competitive equilbrium in the forward market for duration-differentiated energy services? Is the equilibrium efficient, that is, does it maximize social welfare?
\end{problem}
%The (constant) power available in time slot $t$ is  $p_t$,
%and $\VEC p = (p_1,p_2,\ldots,p_T)$ is called the {\em supply profile}. 
%We next consider several versions of the problem of allocating supply (the available power) to demand (the flexible loads).
\section{Adequacy Results}\label{sec:discrete} 
In order to address Problem 1, we start with providing a characterization of the set of supply profiles that are adequate for a given collection of loads.   We then provide a closed-form expression for the minimum amount of power needed to make an inadequate supply adequate. We use these results to identify the optimal   day-ahead and real-time purchase decisions for the supplier.

%In this section, we characterize the set of adequate supply profiles for a given collection of flexible loads.
 %We start with formalizing the notion of adequacy. %For a supply profile $\VEC p$, we define an associated \emph{supply-duration vector} $\VEC s = (s_1,s_2,\ldots,s_T)$ where $\VEC s$ is a non-increasing rearrangement of $\VEC p$ (that is, $\VEC s = \VEC p^{\downarrow}$). 
%We derive conditions that characterize when a supply profile is adequate for a load profile. 

\begin{figure*}[ht]
\centering
\begin{tikzpicture}[yscale=0.25, xscale = 0.165]
\draw [xstep=4,ystep=2, thin, dotted] (0,0) grid (24,10);
\node[anchor=west] at (24,1) {$h_1 = 6$};
\node[anchor=west] at (24,3) {$h_2 = 3$};
\node[anchor=west] at (24,5) {$h_3 = 2$};
\node[anchor=west] at (24,7) {$h_4 = 2$};
\node[anchor=west] at (24,9) {$h_5 = 1$};
\node[anchor=north, rotate=90] at (32,5) {Demand profile $h$};
\node[anchor=east, rotate=90] at (2,0) {$d_1 = 5$};
\node[anchor=east, rotate=90] at (6,0) {$d_2 = 4$};
\node[anchor=east, rotate=90] at (10,0) {$d_3 = 2$};
\node[anchor=east, rotate=90] at (14,0) {$d_4 = 1$};
\node[anchor=east, rotate=90] at (18,0) {$d_5 = 1$};
\node[anchor=east, rotate=90] at (22,0) {$d_6 = 1$};
\node[anchor=north] at (12,-5) {Demand duration $d$};
\draw [fill=blue, fill opacity = 0.2, thick] (0,0) rectangle (24,2);
\draw [fill=green, fill opacity = 0.2, thick] (0,2) rectangle (12,4);
\draw [fill=red, fill opacity = 0.2, thick] (0,4) rectangle (8,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (0,6) rectangle (8,8);
\draw [fill=cyan, fill opacity = 0.2, thick] (0,8) rectangle (4,10);

\draw [xstep=4,ystep=2, thin, dotted] (44-4,0) grid (68-4,10);
\draw [fill=blue, fill opacity = 0.2, thick] (44-4,0) rectangle (68-4,2);
\draw [fill=green, fill opacity = 0.2, thick] (48-4,2) rectangle (56-4,4);
\draw [fill=green, fill opacity = 0.2, thick] (60-4,2) rectangle (64-4,4);
\draw [fill=red, fill opacity = 0.2, thick] (48-4,4) rectangle (56-4,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (48-4,6) rectangle (52-4,8);
\draw [fill=cyan, fill opacity = 0.2, thick] (48-4,8) rectangle (52-4,10);
\draw [fill=yellow, fill opacity = 0.2, thick] (64-4,2) rectangle (68-4,4);
%\node[anchor=north, rotate=90] at (76,5) {Supply profile $p$};
\node[anchor=east, rotate=90] at (46-4,0) {$p_1 = 1$};
\node[anchor=east, rotate=90] at (50-4,0) {$p_2 = 5$};
\node[anchor=east, rotate=90] at (54-4,0) {$p_3 = 3$};
\node[anchor=east, rotate=90] at (58-4,0) {$p_4 = 1$};
\node[anchor=east, rotate=90] at (62-4,0) {$p_5 = 2$};
\node[anchor=east, rotate=90] at (66-4,0) {$p_6 = 2$};
\node[anchor=north] at (56-4,-5) {Adequate supply profile $p$};

%%%%

\draw [xstep=4,ystep=2, thin, dotted] (76-4,0) grid (100-4,10);
\draw [fill=blue, fill opacity = 0.2, thick] (44+28,0) rectangle (64+28,2);
\draw [fill=green, fill opacity = 0.2, thick] (44+28,2) rectangle (56+28,4);
\draw [fill=yellow, fill opacity = 0.2, thick] (56+28,2) rectangle (60+28,4);
\draw [fill=brown, fill opacity = 0.2, thick] (60+28,2) rectangle (64+28,4);
\draw [fill=red, fill opacity = 0.2, thick] (48+28,4) rectangle (56+28,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (48+28,6) rectangle (52+28,8);
\draw [fill=cyan, fill opacity = 0.2, thick] (48+28,8) rectangle (52+28,10);
%\draw [fill=yellow, fill opacity = 0.2, thick] (64+28,2) rectangle (68+28,4);
%\node[anchor=north, rotate=90] at (76,5) {Supply profile $p$};
\node[anchor=east, rotate=90] at (46+28,0) {$p_1 = 2$};
\node[anchor=east, rotate=90] at (50+28,0) {$p_2 = 5$};
\node[anchor=east, rotate=90] at (54+28,0) {$p_3 = 3$};
\node[anchor=east, rotate=90] at (58+28,0) {$p_4 = 2$};
\node[anchor=east, rotate=90] at (62+28,0) {$p_5 = 2$};
\node[anchor=east, rotate=90] at (66+28,0) {$p_6 = 0$};
\node[anchor=north] at (56+28,-5) {Inadequate supply profile $p$};

%%%%%
\end{tikzpicture}
\caption{Characterizing duration-differentiated loads (left), adequate supply profile (center), inadequate supply profile (right).}
\label{fig-demandprofile}
\end{figure*}

\subsection{Adequacy conditions}
Let $p_t$ be the power available  in time slot $t$. The vector $\VEC p = (p_1,p_2,\ldots,p_T)$ is  the \emph{supply profile}. We identify necessary and sufficient conditions under which $\VEC p$ is adequate for the given collection of loads.  Any allocation of supply to loads can be specified by a binary {\em allocation rule} $A \in \{0,1\}^{N \times T} $ where
$A(i,t) = 1$ if and only if load $i$ receives power in slot $t$.  We  define two notions of supply adequacy.
\begin{definition}[Adequacy] {\rm 
The supply profile $\VEC p=(p_1,\cdots,p_T)$ is \emph{adequate} for the demand profile $\VEC h = (h_1,\cdots,h_N)$ if there exists an allocation rule $A(\cdot,\cdot)$ such that 
\[ \sum_t A(i,t) = h_i, \]
\[ \sum_i A(i,t) \leq p_t.\]
If further,  $\displaystyle{\sum_i A(i,t) = p_t}$, 
we will say that $\VEC p=(p_1,\cdots,p_T)$ is  \emph{exactly adequate} for  $\VEC h = (h_1,\cdots,h_N)$.}
\end{definition}

\begin{example}{\rm Consider $T=6$ time slots and $N=5$ flexible loads as illustrated in Figure \ref{fig-demandprofile}. 
If the demand profile is $\VEC h = (1,2,2,3,6)$, the associated demand-duration vector is $\VEC d = (5,4,2,1,1,1)$.  
The supply profile shown in the center panel is exactly adequate to service the loads. The supply profile shown in the right panel has the same total energy, but it is inadequate to service the loads.}
\end{example}

The following lemma is a direct consequence of the above definition. 
\begin{lemma}
If $\VEC p$ is (exactly) adequate for a demand profile $\VEC h$, then any temporal rearrangement of $\VEC p$ is also (exactly) adequate for the same demand profile $\VEC h$.
\end{lemma}
We will characterize adequacy more directly via the demand-duration vector. 
For this we employ some notions from majorization theory.

\begin{definition}[Majorization]{\rm \label{def:majorization}
Let $\VEC a = (a_1,\cdots,a_T)$ and $\VEC b = (b_1,\cdots,b_T)$ be two non-negative  vectors. Denote by $\VEC a^{\downarrow}, \VEC b^{\downarrow}$ the non-increasing rearrangements of $\VEC a$ and $\VEC b$ respectively. 
%(that is, $a^{\downarrow}_t \geq a^{\downarrow}_{t+1}$).
We say that $\VEC a$ majorizes $\VEC b$, written $\VEC a \lessthan \VEC b$, if 
\bromalist
\item $\sum_{s=t}^T a^{\downarrow}_s \leq \sum_{s=t}^T b^{\downarrow}_s$, for $t=1,2,\ldots,T$, and 
\item $\sum_{s=1}^T a^{\downarrow}_s= \sum_{s=1}^T b^{\downarrow}_s$.
\end{list}
If only the first condition holds, we say that $\VEC a$ weakly majorizes $\VEC b$, written 
$\VEC a \lessthan^{w} \VEC b$.}
\end{definition}

\begin{remark}{\rm The inequalities in our definition of majorization are reversed from standard use in majorization theory. 
This departure from convention allows us to write our adequacy conditions
as $\VEC d \lessthan \VEC p$ and $\VEC d \lessthan^w \VEC p$  which suggests the intuitive adequacy condition of demand being ``less than'' supply .}
\end{remark}
%Define $d_t := \sum_i\mathds{1}_{\{t \leq h_i\}}$ and $\VEC d := (d_1,d_2,\ldots,d_T)$. $\VEC d$ is  the demand-duration vector associated with the demand profile $(h_1,h_2,\ldots,h_N)$.  Note that $\VEC d = {\VEC d}^{\downarrow}$.
Our next result characterizes adequacy.

\begin{theorem}[\sc Adequacy]\label{thm:two}
\balphlist
\item The supply profile $\VEC p$  is exactly adequate for a demand profile $\VEC h$ with the associated demand-duration vector $\VEC d$ if and only if $\VEC d \lessthan \VEC p$.
\item The supply profile $\VEC p$  is adequate for a demand profile $\VEC h$ with the associated demand-duration vector $\VEC d$ if and only if 
 $\VEC d \lessthan^{w} \VEC p$.
% Let $\Delta = \sum_t p_t - \sum_i h_i$. Define $d^{\Delta}_t := d_t + \Delta\mathds{1}_{\{t \leq 1\}}$.   Then,   $\VEC p$ is simply adequate if and only if \\
 %(a) $\Delta \geq 0$ and (b) $\VEC p \morethan \VEC d^{\Delta}$.
 \end{list}
\end{theorem}
\proof{Proof}
 See Appendix \ref{sec:two}.
\endproof
\subsection{Least Laxity Allocation}

We now describe an allocation rule that will play a key role in this paper.
Given an allocation rule $A$, we define the laxity of load $i$ at time $t$ as $x_i(t) := T-t+1 - \left(h_i -\sum_{s=1}^{t-1}A(i,s)\right)$. 

\begin{definition}[LLF Allocation]{\rm  \label{defn:LLF}
Fix the supply profile $\VEC p = (p_1,p_2,\ldots,p_T)$. The {\em Least Laxity Allocation} rule $A(i,t)$ is defined by
 \bromalist
  \item At time $1$, $x_i(1) = T-h_i$. Arrange the loads in non-decreasing order of $x_i(1)$ and let $\mathcal{A}_1$ be the collection of the first $p_1$ loads from this order. Set $A(i,1) =1$ if and only if $i \in \mathcal{A}_1$.
  \item At time $t$,  $x_i(t) = T -t+1-\left(h_i -\sum_{s=1}^{t-1}A(i,s)\right)$. Arrange loads in non-decreasing order of $x_i(t)$ and let $\mathcal{A}_t$ be the collection of the first $p_t$ loads from this order. Set $A(i,t) =1$ if and only if $i \in \mathcal{A}_t$.
 \end{list}}
\end{definition}

As its name suggests, at each time $t$ LLF  gives  priority to loads with smaller laxity.
Our next result shows that the LLF allocation successfully services the loads when the supply profile is adequate.  
We have:

\begin{theorem}\label{thm:three}
 If the supply profile $\VEC p = (p_1,p_2,\ldots,p_T)$ is adequate, 
 then the Least Laxity First allocation rule satisfies all the demands, i.e. 
 \[ \sum_t A(i,t) = h_i, \quad \sum_i A(i,t) \leq p_t \]
\end{theorem}
\proof{Proof}
See Appendix \ref{sec:app_3}.
\endproof

%\textbf{Remark 1} \
%LUDF bears a family resemblance to several  scheduling algorithms proposed to match flexible loads to an inflexible supply, including
%EDF (earliest deadline first), LLF (least laxity first), ... \textbf{TO BE COMPLETED}

%\section{Supply Uncertainty and Recourse Decisions}
\subsection{Supplemental Power Purchases}
%In the above analysis the forecast of free supply $\VEC p$ is assumed to be accurate. One possible way to make this forecast is as follows. Given a statistical model for the free supply, the forecast vector $\VEC p$ is defined such that the true realization of the free supply majorizes $\VEC p$ with probability $\alpha$.  Formally, if $\VEC Q$ is the random vector denoting the free supply and $\mathds{P}$ is the probability distribution of $\VEC Q$,  $\VEC p$ is defined as a solution of the following equation
%\begin{equation}
%\mathds{P} ( \VEC Q \morethan^w \VEC p) \geq \alpha .
%\end{equation}
%If the contracts in the forward market are chosen based on $\VEC p$, then with probability at least $\alpha$ the  realization  $\VEC Q$ (including any scheduled conventional generation) will be adequate for the chosen contracts. If $\VEC Q$ is inadequate, the supplier must purchase additional power in real-time.  
It may happen that the supply profile is not adequate for a given demand profile. In this case, the supplier will have to purchase additional power to serve the loads.  We determine the least costly increment in supply profile to make it adequate.
We consider two scenarios: (a)  {\em Oracle information:} the entire supply profile $p$ is revealed in advance, (b)  
{\em Run-time information:} the power available in slot $[t,t+1)$ is revealed at time $t$, i.e. immediately before the beginning of the slot. 

\textbf{Case (a):} \ The supplier needs to serve a demand profile $\VEC h$ with the associated demand-duration vector $\VEC d =(d_1,d_2,\ldots,d_T)$. Before the time of delivery, the supplier learns the true realization of the entire supply profile $\VEC p=(p_1,\ldots,p_T)$. If $\VEC d \lessthan^w \VEC p$,  the supply is adequate and there is no need for supplemental power. In the case of inadequate supply, the additional power to be purchased at minimum cost while ensuring that all demands are met is given by the solution of the following optimization problem:
%\emph{Optimal Recourse Decision Problem}
\begin{equation}
    \min_{\VEC a \geq 0} \sum_{t=1}^T c \cdot a_t \notag \quad
    \mbox{subject to~~~} \VEC d \lessthan^w (\VEC p + \VEC a), \label{LP}
\end{equation}
where $c \geq 0$ is the unit price of supplemental power.  This is a linear programming problem since the majorization inequalities are linear.


\textbf{Case (b):}\  The power available in each slot is revealed just before the beginning of that slot. The supplier now faces  a sequential decision-making problem where the information available to make the purchase decision $a_t$ at time $t$ is $\VEC d, p_1,p_2,\ldots,p_t$. %Note that $t$ here is the real time and we are \emph{not} assuming that time indices have been reordered to ensure monotonicity of supply profile. 
The supplier's objective  is to minimize the total cost of  additional power $\sum_{t=1}^Tc\cdot a_t$ while ensuring that all load demands are met.

%It is clear that the  supplier's total cost in this scenario can be no less than the cost under Case A considered above (see Theorem \ref{thm:procurement}). 
Clearly the supplier's optimal cost in Case (b) is lower bounded by its optimal cost in Case (a). Surprisingly, it happens that the
optimal costs and corresponding decision strategies are identical in both situations. More precisely, we have:

\begin{figure*}[ht]
\begin{theorem}\label{thm:procurementb}
Consider the following decision strategy for the supplier: \\
(i) The additional power purchased at  $t=1$ is $a_1 = (d_T-p_1)^+$. The total power $(p_1+a_1)$ is allocated to consumers according to the LLF policy described in Definition \ref{defn:LLF}.\\
(ii) At time $t$, knowing the supply $p_1,p_2,\ldots,p_t$ and the purchases $a_1,\ldots,a_{t-1}$, the power purchased $a_t$ is the solution of the following optimization problem:
\begin{align} \nonumber
 &\min_{a_t} a_t  \\
 s.t.~~&(p_1+a_1,p_2+a_2,\ldots,p_{t-1}+a_{t-1},p_t+a_t) \morethan_w (d_{T-t+1},d_{T-t+2},\ldots,d_T)
\end{align}
The total power $(p_t+a_t)$ is allocated to consumers according to the LLF policy.  Then,
\balphlist
\item 
This strategy is optimal under both the oracle information and run-time information cases. 
\item The optimal cost is $c\left( \max_{t} \left(\sum_{ s \geq t} (d_s -p^{\downarrow}_s)\right)^+\right)$.
\end{list}
\end{theorem}

\end{figure*}
\proof{Proof}
See Appendix \ref{sec:procurementb}.
\endproof


%%%%%%
%\begin{figure}[h]
%\centering
%\includegraphics[width=3.5in]{Figures/supplyCM.pdf}
%\caption{Characterizing market outcomes.}
%\label{fig-flow}
%\end{figure}


%%%%%% 

\section{The supplier's optimization problem}\label{sec:supplier_problem}
We can now address Problem 1 described in Section~\ref{sec:PF}.  Suppose the supplier purchases a power profile $\VEC y = (y_1,y_2,\ldots,y_T)$ in the day-ahead market. In real-time, the renewable supply takes a realization $\VEC r$, so that the total realized supply profile is $\VEC p = \VEC r+ \VEC y$. Since, this supply may not be adequate, the supplier would have to purchase real-time energy. The optimal policy for making these real-time purchases is given by  the decision strategy described in Theorem~\ref{thm:procurementb} with the associated cost given as $c\left( \max_{t} \left(\sum_{ s \geq t} (d_s -p^{\downarrow}_s)\right)^+\right)$. Hence, the supplier's total expected cost is given as
\begin{align} \label{eq:expected_cost2}
J(\VEC y) = c^{da}\sum_{t=1}^T y_t + c^{rt}\mathds{E}\Bigg[  \max_{t} \left(\sum_{ s \geq t} (d_s -(\VEC R + \VEC y)^{\downarrow}_s)\right)^+\Bigg],
\end{align}
where the expectation is over the renewable supply $\VEC R$. The supplier's optimization problem now is to choose $\VEC y$ to minimize $J(\VEC y)$. Recall that $\VEC y$ is discrete-valued. However, by relaxing the integer constraint on $\VEC y$, we get a convex optimization problem which can be used to provide approximate solutions to supplier's optimization problem.
\begin{theorem}\label{thm:convexity}
If we relax the constraint that $\VEC y$ can take only integer values, then the supplier's objective function is convex in $\VEC y$.
\end{theorem}
\begin{proof}
See Appendix \ref{sec:convexity}.
\end{proof}
%\section{Rate-constrained energy services} 
%
%We have thus far assumed that consumers demand $1$ kW for a specified number of time slots.
%We now consider a more general energy service, which provides a specified quantity of energy to be delivered over $T$ time slots. However, the power level in each time slot can assume any integer value up to a maximum  rate $m$.  
%We will argue that these products can be viewed as a combination of the  duration-differentiated services  at a fixed power level of $1$ kW presented before. 
%
%Consumer $i$ specifies two quantities: $(E_i,m_i)$, $E_i$ is the total energy to be consumed over $T$ time slots at a maximum rate of $m_i$ kW per time slot. Both $E_i$ and $m_i$ are integer-valued. 
%For example, a consumer specifying $(100,10)$ requires $100$ kW-slots of energy with the constraint that the consumption rate in each time slot is $0,1,2,\ldots$ or $10$ kW. A consumer specifying $(E_i,m_i)$ is satisfied with any supply allocation $A_t \in \{0,1,\ldots,m_i\}$ such that $\sum_t A_t = E_i$. The consumer model of section \ref{sec:discrete} corresponds to the case where $m_i =1$. 
%
%Consider a consumer whose energy requirement and rate constraint are specified by the pair $(E,m)$. Let $k,r$ be such that $E = km + r$ with $r <m$. The following result shows that for the purpose of allocating supply, a consumer specifying $(E,m)$ is equivalent to a collection of $m$ consumers with $(E_n = k+1, m_n =1)$ for $n=1,2,\ldots,r$ and $(E_n = k,m_n=1)$ for $n=r+1,\ldots,m$. Hence, the adequacy and allocation results of Section \ref{sec:discrete} (which were derived for consumers with $m=1$) can be used for the variable rate consumers as well.
%
%\begin{theorem}\label{thm:var_rate}
% Consider a consumer whose energy requirement and rate constraint are specified by the pair $(E,m)$. Let $k,r$ be such that $E = km + r$ with $r <m$. Then, a supply allocation satisfies
% \begin{equation}\label{eq:var_rate1}
%  A_t \in \{0,1,\ldots, m\} \quad \sum_t A_t =E
% \end{equation} 
% if and only if 
% \begin{equation} \label{eq:var_rate2}
% A_t = \sum_{n=1}^m A^n_t,
% \end{equation}
% where $A^n_t \in \{0,1\}$ and $\sum_t A^n_t =k+1$ for $n\leq r$ and $\sum_t A^n_t = k$ for $n>r$.
%\end{theorem}
%\proof{Proof.}
%See Appendix \ref{sec:var_rate}.
%\endproof
%%If we impose that $k_n$ is an integer and $E_n$ is a multiple of $k_n$, $E_n=\alpha_n k_n$ hence a $(E_n,k_n)$ product can be characterized in terms of



==> 03marketsNewEx.tex <==
\section{Forward market for duration-differentiated contracts}\label{sec:market}
%%NEW TEXT
In the analysis presented in the previous sections, the set of duration-differentiated  loads was assumed to be fixed. In this section the problem of arriving to that fixed set is investigated. We consider the case in which the fixed set of duration-differentiated loads is the outcome of a market interaction between consumers and suppliers. 

In particular, we consider a forward market for duration-differentiated services and investigate its properties. Duration-differentiated services couple supply and consumption across different time slots. A natural way to capture this is to consider a forward market for the whole operational period where services of different durations are bought and sold. In this way, both consumers and suppliers can effectively quantify the value/cost of consuming/producing these services.  All the market transactions are completed before the delivery time. Thus, the market decisions are made prior to the operational decisions required for the delivery of the products which is a characteristic of direct load control. In order to illustrate the advantages of forward markets, we perform a comparison with a stylized real-time spot market implementation. The results shed light about potential inefficiencies resulting from the implementation of spot markets in which the inter-temporal dimension of duration-differentiated contracts is hard to capture.

% The forward market has three elements:
%
%\balphlist
%\item Services: The services are differentiated by the number $h$ of time slots within $T$ slots during which 1 kW of electric power is delivered.  Service $h$ is sold at price $\pi(h)$.
%\item Consumers: The benefit to a consumer who receives $h$ slots is  $U(h)$; all consumers have the same utility function $U$. 
%\item Supplier: The supplier receives for free the power with profile $\VEC R = (R_1, \cdots, R_T)$.  The supplier knows the profile $\VEC p$.  The supplier may purchase additional energy $\VEC y$ with total cost  $J(\VEC y)$ as defined in the previous section.
%\end{list}
%, $\VEC h = (h_1,h_2,\ldots,h_N)$ in which $h_i$ represents the duration that consumer $i$ is receiving,

In order to make the analysis tractable, we focus on idealized markets structures and consumers and suppliers behaviors. In particular, we assume the following:
\begin{enumerate}
\item Competitive Market: Suppliers and consumers are assumed to be price takers without the possibility of impact the market prices.
\item Certainty Equivalence: In order to make their market decision, the suppliers ignore the uncertainty in their forecast by treating their expected value of renewable power as the true realization. 
\end{enumerate}
The first assumption is standard in market analysis in which price are assumed to be exogenous to the players decisions. The second assumption allows to simplify the suppliers problem in the market setting. It avoids the need to consider the costs resulting from the two-stage optimization problem presenting previously. By assuming this, the additional power cost will be just $c^{da} \sum_{t=1}^T y_t$.
%Certainly, this assumption relies on the quality of the forecast available by the suppliers which for the case of solar power is.




The information flow of the market is depicted in Figure \ref{fig-flow}. Facing a menu of services with associated prices $\mathcal{M}=\{k,\pi(k)\}$, consumer $n$ selects a service $h_n$ that maximizes her net benefit, while the supplier selects the number $n_t$ of services of duration $t$  to produce that  maximize her net profit.  

\begin{figure*}[ht]
\centering
\usetikzlibrary{shapes.arrows,fadings}
\begin{tikzpicture}[scale=0.4]
\draw [fill=blue, fill opacity = 0.2] (4,-1) rectangle (14,2);
\draw [fill=green, fill opacity = 0.2] (2,5) rectangle (16,9);
\draw [fill=red, fill opacity = 0.2] (0,12) rectangle (2,14);
\draw [fill=red, fill opacity = 0.2] (4,12) rectangle (6,14);
\draw [fill=red, fill opacity = 0.2] (8,12) rectangle (10,14);
\draw [fill=red, fill opacity = 0.2] (16,12) rectangle (18,14);
\node[] at (1,13) {$h_1$};
\node[] at (5,13) {$h_2$};
\node[] at (9,13) {$h_3$};
\node[] at (13,13) {$\cdots$};
\node[] at (17,13) {$h_N$};
\node[] at (9,7) {\fontsize{14}{16} ${\cal M} = \{k,\pi(k)\}$};
\node[] at (9,0.5) {$(n_1, n_2, \cdots, n_T)$};
\node [
    fill=red!60!black,
    fill opacity=0.7,
    single arrow,
    minimum height=0.5cm,
    single arrow head extend=0.15cm,
    rotate=90
] at (6,3.5){};
\node [
    fill=red!60!black,
    fill opacity=0.7,
    single arrow,
    minimum height=0.5cm,
    single arrow head extend=0.15cm,
    rotate=270
] at (12,3.7){};
\node [
    fill=red!60!black,
    fill opacity=0.7,
    single arrow,
    minimum height=0.5cm,
    single arrow head extend=0.15cm,
    rotate=90
] at (6,10){};
\node [
    fill=red!60!black,
    fill opacity=0.7,
    single arrow,
    minimum height=0.5cm,
    single arrow head extend=0.15cm,
    rotate=270
] at (12,10.2){};
\end{tikzpicture}
\caption{Market implementation.}
\label{fig-flow}
\end{figure*}
%%%This paragraph has changes
We first characterize the decisions that maximize total social welfare, defined as aggregate consumer utility minus the cost of  purchased energy.  We then show that the optimum decisions can be sustained as a  competitive equilibrium. Lastly,   we compare the competitive equilibrium in a real-time spot market with
the equilibrium for our duration-differentiated forward market. 
%As presented, the spot market equilibrium allocation can lead to a reduced social welfare.
%and the spot prices can exhibit greater volatility. 

\subsection{Social Welfare Problem}
We consider a set of homogenous consumers, consumer $i=1,\ldots,N$ enjoys utility $U(h)$ upon consuming 1 kW of power for  $h$ slots. The supplier has available for free a quantity of power with profile $\VEC r = (r_1,\ldots,r_T)$, and can also purchase additional energy at $c^{da}$ per kW-slot. %Given that usually $\VEC p$ will represent some renewable power supply over the operational periods, we assume that the supplier have information about the ordered profile ${\VEC p} ^{\downarrow}$.
 The  social welfare  optimization problem is
%Consequently, the previous cost function $g_j(x_j)$ can be defined by $g_j(x_j)=c(x_j-p_j)^+$ and
\begin{align}
    &\max_{\VEC h \geq 0,\VEC y \geq 0} \sum_{i=1}^N U(h_i) - \sum_{t=1}^T c^{da} y_t \notag \\
    & \mbox{subject to~} 
     d_t = \sum_{i=1}^N \mathds{1}_{\{t\leq h_i\}} \notag \\
    & \hspace{55pt}\VEC y + \VEC r   \morethan^w \VEC d \notag 
\end{align}

%\begin{remark}{\rm 
%Since $\sum_{i=1}^N U(h_i) = \sum_{t=1}^{T-1} U(t)[d_t-d_{t+1}] + U(T)d_T$, this  is a linear integer programming problem.  It may
%therefore be surprising that in case $U(h)$ is convex or concave, its solution coincides with that of the LP problem obtained by relaxing the integer constraints.}
%\end{remark}

%\begin{remark}{\rm 
%Since the supplier knows ${\VEC p} ^{\downarrow}$ but not the profile $\VEC p$, the additional supply $\VEC y$ does not represent a chronological ordered profile but a supply-duration vector. }
%\end{remark}


%%%%for one column
\begin{figure*}[ht]

\begin{theorem}[\sc Social Welfare] \label{thm:soc_welfare} 
Assume the profile $\VEC r$ is arranged in decreasing order: $\VEC r = {\VEC r}^{\downarrow}$.
%\setlength{\leftmargini}{0.15in}
\balphlist
\item (Convex utility)  Suppose $U(h) - U(h-1)$ is a non-negative, non-decreasing function of $h$ (with $U(0)=0$) and the number of consumers $N$ is larger than $r_1$.  Define
\begin{equation}\label{eq:convex_kstar}
k^* = \left\{ \begin{array}{ll}
	\min k : k \in \{0,1,\ldots,(T-1)\}, \ \ \frac{U(T)-U(k)}{T-k} \geq c^{da} & \text{if this exists} \\
	T & \text{otherwise} \end{array} \right.
\end{equation}
	
%Let $k^*$ be the least  $k \in \{0,1,\ldots,(T-1)\}$ for which
%\begin{equation}
%\frac{U(T)-U(k)}{T-k} \geq C .
%\end{equation}
%If such a value does not exist, take $k^*=T$. 
If  $k^* \geq 1$, the optimum demand duration  is
\begin{align}
d^*_t =\left \{\begin{array}{ll} r_t &\mbox{ if $t < k^*$}\\
                                      r_{k^*} &\mbox{ if $t \geq k^*$} \\                           
                                        \end{array}
                                       \right. \label{eq:soc_welfare1a}
\end{align}    
If $k^* =0$, the optimum demand duration vector is $d^*_t =N$ for all $t$.

\item (Concave utility)  Suppose $U(h)- U(h-1)$ is a non-negative, non-increasing function of $h$ (with $U(0)=0$) and the number of consumers $N$ is larger than $\sum_t r_t$. Define
\begin{equation}\label{eq:concave_kstar}
k^* = \left\{ \begin{array}{ll}
	\min k : k \in \{1,\ldots,T\}, \ \ {U(k)-U(k-1)} \geq c^{da}  & \text{if this exists} \\
	0 & \text{otherwise} \end{array} \right.
\end{equation}
%
%Let $k^*$ be the largest $k \in \{1,\ldots,T\}$ for which
%\begin{equation}
%{U(k)-U(k-1)} \geq C .
%\end{equation}
%If such a value does not exist, take $k^*=0$.
If $k^* \geq 1$, the optimum demand duration   is  
\begin{align}
d^*_t =\left \{\begin{array}{ll} N &\mbox{ if $t \leq k^*$}\\
                                      0 & \mbox{ if $t > k^*$}\\
                                        \end{array}
                                       \right. \label{eq:soc_welfare1b}
\end{align} 
If $k^*=0$, the social welfare maximizing demand duration vector is  
\begin{align}
d^*_t =\left \{\begin{array}{ll} 
                                      \sum_{i=1}^T r_i &\mbox { if $t=1$} \\
                                      0  &\mbox{ if $t > 1$}\\
                                        \end{array}
                                       \right. \label{eq:soc_welfare1c}
\end{align} 
%The optimal supply-duration vector of additional supply needed is $\VEC y^* = \VEC d^* - \VEC p$.
\end{list}                 
\end{theorem}

\end{figure*}

\proof{Proof}
See Appendix \ref{sec:soc_welfareproof}.
\endproof

In the convex case, the utility increments are non-decreasing in $h$ and the optimal allocation   favors longer duration contracts. In the concave case,  the utility increments are non-increasing in $h$ and the optimal  allocation   favors the shortest durations. 

\begin{remark}{\rm 
In standard commodity markets, the usual setting is to consider concave utility functions which reflects the decreasing marginal utility of many goods. In the case of duration-differentiated loads, the concave case could represent situations in which additional hours of consumption does not increase the marginal utility, for example the filtering of a pool beyond the minimum numbers of hours. However, in this case convex utility functions are also of interest. That could represent loads for which interruptions of the consumption is material. Examples include industrial mining processes, power supply for computational applications, air flow in hospitals.}
\end{remark}

\begin{example}{\rm 
For example, take  $\VEC r=(5,4,2,1,1,0)$, the number of consumers $N=14$ and the time period $T=6$. In addition, the utility function for the convex case is such that
\begin{equation}
%\frac{U(6)-U(5)}{1} \geq c^{da} .
{U(6)-U(5)} \geq c^{da} .
\end{equation}
and for the concave case
\begin{equation}
{U(1)-U(0)} \geq c^{da} .
\end{equation}
In the convex case the optimal allocation is is $\VEC h=(1,2,2,3,6)$ as in Figure \ref{fig-ex1} (left). Note that an additional unit of supply is utilized and used to create a contract of duration 6 hours. In the concave case only contracts of duration 1 slots are required as in Figure \ref{fig-ex1} (middle). Note that in this case, also an additional unit of supply is utilized to create an additional contract of duration 1.}
\end{example}

% is such that  large that additional supply is not purchased.  In the convex case the optimal allocation is 
%is $\VEC h=(1,2,2,3,5)$ as  in Fig \ref{fig-ex1} (left).   In the concave case only contracts of duration 1 slots are required as in Fig \ref{fig-ex1} (middle).  

%\begin{figure*}[h]
%\centering
%%\includegraphics[width=4.5in]{Figures/convex-concave.png}
%\includegraphics[width=5in]{Figures/Ex2.pdf}
%\caption{Optimal allocation for convex case (left), concave case (middle), number of interruptions (right).}
%\label{fig-ex1}
%\end{figure}

\begin{figure*}[ht\begin{figure*}]
\centering
\begin{tikzpicture}[scale=0.25]
\draw [xstep=2,ystep=2, thin, dotted] (0,0) grid  (12,10);
\node[anchor=east] at (0,1) {$h_1 = 6$};
\node[anchor=east] at (0,3) {$h_2 = 3$};
\node[anchor=east] at (0,5) {$h_3 = 2$};
\node[anchor=east] at (0,7) {$h_4 = 2$};
\node[anchor=east] at (0,9) {$h_5 = 1$};
%\node[anchor=north, rotate=90] at (30,5) {Demand profile $h$};
%\node[anchor=east, rotate=90] at (2,0) {$d_1 = 5$};
%\node[anchor=east, rotate=90] at (6,0) {$d_2 = 4$};
%\node[anchor=east, rotate=90] at (10,0) {$d_3 = 2$};
%\node[anchor=east, rotate=90] at (14,0) {$d_4 = 1$};
%\node[anchor=east, rotate=90] at (18,0) {$d_5 = 1$};
%\node[anchor=east, rotate=90] at (22,0) {$d_6 = 1$};
\node[anchor=north] at (6,0) {$d =(5,4,2,1,1,1)$};
\draw [fill=blue, fill opacity = 0.2, thick] (0,0) rectangle (12,2);
\draw [fill=green, fill opacity = 0.2, thick] (0,2) rectangle (6,4);
\draw [fill=red, fill opacity = 0.2, thick] (0,4) rectangle (4,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (0,6) rectangle (4,8);
\draw [fill=cyan, fill opacity = 0.2, thick] (0,8) rectangle (2,10);

\draw [fill=blue, fill opacity = 0.2, thick] (22,0) rectangle (24,2);
\draw [fill=green, fill opacity = 0.2, thick] (22,2) rectangle (24,4);
\draw [fill=red, fill opacity = 0.2, thick] (22,4) rectangle (24,6);
\node[] at (23,8) {$\vdots$};
\node[] at (23,11) {$\vdots$};
\node[] at (20,9) {$h_i = 1$};
\draw [fill=violet, fill opacity = 0.2, thick] (22,12) rectangle (24,14);
\draw [fill=yellow, fill opacity = 0.2, thick] (22,14) rectangle (24,16);
\draw [fill=cyan, fill opacity = 0.2, thick] (22,16) rectangle (24,18);
\node[anchor=north] at (23,0) {$d =(14,0,0,0,0,0)$};

\draw [xstep=2,ystep=2, thin, dotted] (34,0) grid (46,10);
\draw [fill=blue, fill opacity = 0.2, thick] (34,0) rectangle (46,2);
\draw [fill=green, fill opacity = 0.2, thick] (34,2) rectangle (40,4);
\draw [fill=red, fill opacity = 0.2, thick] (34,4) rectangle (36,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (34,6) rectangle (36,8);
\draw [fill=red, fill opacity = 0.2, thick] (38,4) rectangle (40,6);
\draw [fill=yellow, fill opacity = 0.2, thick] (38,6) rectangle (40,8);
\draw [fill=cyan, fill opacity = 0.2, thick] (34,8) rectangle (36,10);
\node[anchor=north] at (40,0) {$q =(5,2,4,1,1,1)$};

\end{tikzpicture}
\caption{Optimal allocation for convex case (left), concave case (middle), number of interruptions in the convex case (right).}
\label{fig-ex1}
\end{figure*}

\subsection{Competitive equilibrium}
%CHANGES
We now analyze a stylized forward market for the production and consumption of duration-differentiated services. We focus on a perfect-competition setting in which prices are assumed to be \textit{exogenous} to the players' decisions. Consequently, all players are \textit{price takers}, i.e., they cannot influence the prices. The perfect-competition setting is certainly an idealization but it provides valuable insights in terms of market design. In particular, these outcomes are usually used as a benchmark for analysis in which perfect-competition is not considered, e.g., monopolistic or oligopolistic settings. %Recognizing the stylized market that we consider, the design does capture a key element of the duration-differentiated products: inter-temporal considerations. As we will present in the comparison with a spot-market, this inter-temporal dimension drives the efficiency gains associated with the forward market.  

The market determines a price for each service, every consumer selects the service she wants to maximize her net benefit, and the supplier decides how much of each service to produce. If the demand and supply for each service match, a competitive equilibrium is said to exist. Mathematically, a competitive equilibrium is defined as follows. 

\begin{definition}[Competitive Equilibrium]{\rm
The supplier's  service production vector $\VEC n = (n_1,n_2,\ldots,n_T)$, the consumers'  demand  profile $\VEC h = (h_1,h_2,\ldots,h_N)$, and a set $\{\pi(h)\}$ of prices  constitute a {\em competitive equilibrium} if  three conditions hold:
\bromalist
\item Consumer Surplus Maximization: $h_i \in \argmax_h U(h) - \pi(h)$, all $i$.
\item Profit Maximization: The services produced maximize profit, i.e. $\VEC n$ solves this optimization problem:
\begin{align}
    &\max_{\VEC n \geq 0,~ \VEC y \geq 0}  \sum_{t=1}^{T}(n_t\pi(t) - Cy_t)  \notag \\
    & \mbox{subject to~} d_t = \sum_{i=t}^T n_i \notag \\
     & \hspace{20pt} \VEC r + \VEC y \morethan^w \VEC d \notag 
\end{align}
\item Market Clearing: The  supply and demand for each service are equal: $n_t = \sum_{i=1}^N \mathds{1}_{\{h_i=t\}}$.
\end{list}}
\end{definition}

\begin{definition}[Efficiency]{\rm
The competitive equilibrium is {\em efficient} if the resulting allocation maximizes social welfare.}
\end{definition}

We next characterize efficient competitive equilibria for convex and concave utility functions.

\begin{theorem}[\sc Efficient Competitive Equilibrium] \label{thm:market} 
Assume the profile $\VEC r$ is arranged in decreasing order: $\VEC r = {\VEC r}^{\downarrow}$.
%\setlength{\leftmargini}{0.15in}
\balphlist
\item (Convex utility)  Suppose  $U(h)-U(h-1)$ is non-decreasing  (with $U(0)=0$) and the number of consumers $N$ is larger than $r_1$. Then an efficient competitive equilibrium exists and  is described as follows: \\
Prices: $\pi(h)=U(h)$. \\
Supplier's production: Define $k^*$ as in \eqref{eq:convex_kstar}. Then,  if $k^* \geq 1$, $n_t=r_t-r_{t+1}$ for $t<k^*$, $n_t = 0,$ for $k^* \le t <T$, and $n_T=r_{k^*}$ %in which 
%$k^*$ is the least $k \in \{0,1,\ldots,(T-1)\}$ for which
%\begin{equation}
%\frac{\pi(T)-\pi(k^*)}{T-k^*} \geq C . \label{6}
%\end{equation}
%If such a value does not exist, take $k^*=T$. 
If $k^* =0$, the supplier's production is $n_T=N$.\\
Consumption: $n_t$ consumers purchase duration $t$ service, so market is  cleared.\\
\item (Concave utility)  Suppose $U(h)- U(h-1)$ is non-increasing (with $U(0)=0$) and the number of consumers $N$ is larger than $\sum_t r_t$. Then an efficient competitive equilibrium exists and  is described as follows: \\
 Prices: $\pi(h)=\min(c^{da},U(1))h$.\\
Supplier's production:  Define $k^*$ as in \eqref{eq:concave_kstar}. If $k^* \geq 1$, $n_{k^*}=N$ 
%in which $k^*$ is the largest $k \in \{1,\ldots,T\}$ for which
%\begin{equation}
%{U(k)-U(k-1)} \geq C . \label{7}
%\end{equation}
If $k^*=0$,  $n_1=\sum_t r_t$ and $n_k=0$ for $k>1$.\\
Consumption:  $n_t$ consumers purchase duration $t$ service, so market is cleared.
%\item In both cases, the equilibrium is efficient. 
\end{list}
\end{theorem}

%\begin{proof}
%{See Appendix \ref{sec:market_proof}}.
%\end{proof}
\proof{Proof} See Appendix \ref{sec:market_proof}. \endproof

\begin{remark}{\rm In essence, Theorem \ref{thm:market} is reminiscent of the first fundamental theorem of welfare economics \cite{mascolell} which states that under certain conditions competitive equilibria are Pareto efficient. Note that our market model differs from the standard market models since each consumer faces a discrete choice \cite{indivisible}.  Further, Theorem \ref{thm:market} is constructive in the sense that it identifies an equilibrium price vector.}\end{remark}

%\begin{remark}{\rm In essence, Theorem \ref{thm:market} is reminiscent of the first fundamental theorem of welfare economics \cite{mascolell} which states that under certain conditions competitive equilibria are Pareto efficient. Note that our market model differs from the standard models since each consumer faces a discrete choice.  Further, Theorem \ref{thm:market} is constructive in the sense that it identifies an equilibrium price vector. }\end{remark}

\begin{remark}{\rm In the above analysis, the supply side represents an aggregation of many suppliers. Note that  individual price taking suppliers may benefit by coordinating to offer longer service contracts in order to take advantage of higher prices for longer durations. We assume that the suppliers are able to identify and exploit all such opportunities. We further assume that even with such coordination the number of effective suppliers is large enough to justify the assumption of a competitive market. 
}
\end{remark}

\begin{remark}{\rm In the convex case, the marginal price of the $h$th slot, $\pi(h) - \pi(h-1)$ is \textit{increasing}.  This is due to the fact that from a given 
supply profile it may be possible to produce  a $m$-slot and a $k$-slot service but not a $(m+k)$-slot service, as can be seen from the definition of adequacy.  This contrasts with the assumption in  \cite{Chao-Oren86} that, for conventional generator technology, the marginal price of producing electricity for slot $h$ decreases with $h$. In the concave case above this issue does not arise since service of a single duration is produced.}
\end{remark}

\begin{remark}{\rm 
%An $h$-slot service purchased by a customer need not be delivered contiguously: there may be service interruptions.    Consider the convex case and suppose $C$ is so large that $k^* = T$ in \eqref{6} and the services produced by the supplier are
%given by $n_t = r_t -r_{t+1}$.  
Suppose the actual chronological profile of the power is $\VEC q = (q_1, \cdots, q_T)$.
%(so $\VEC p = \VEC q^{\downarrow}$).  
%$\VEC q$
Suppose $\VEC q$ has $(m+1)$ local minima.  Then, in the market allocations in the convex case, each service will have at most $m$ interruptions.  For the same example as before Figure \ref{fig-ex1} (right) shows that there is
at most one interruption since $\VEC q = (5,2,4,1,1,1)$ has two local minima.}
\end{remark}

\subsection{Real-time  vs duration-differentiated markets}
We compare the duration-differentiated market with a real-time spot market that operates as follows.  At the beginning of slot $t$ the market determines a price $\pi_t$ for 1kW of power delivered during slot $t$. The price $\pi_t$ equates the supply function $s_t(\pi)$ and demand function $q_t(\pi)$, i.e., $s_t(\pi_t) = q_t(\pi_t)$.  We model these functions.  The supply function is straightforward.  At the beginning of slot $t$, the supplier receives for free power $r_t$ and offers it for sale inelastically.  She can also supply as much power as she wishes at price $C$ per kW-slot.  Thus the supply function is
\begin{equation} \label{a1}
s(\pi) =
\left \{
\begin{array} {ll}
\infty & \mbox{ if } \pi > c^{rt} \\
\mbox{$[p_t,\infty)$} & \mbox{ if } \pi =c^{rt}  \\
p_t & \mbox{ if } \pi < c^{rt}
\end{array}
\right .
.
\end{equation}
The demand function is a bit more complicated.  At the beginning of slot $t$, consumer $n$ determines her willingness to pay $v_n(t)$ for 1 kW in slot $t$. So the (aggregate) demand function is
\begin{equation} \label{a2}
q_t(\pi) = \sum_{i=1}^N \mathds{1}_{\{\pi \le v_n (t)\}}.
\end{equation}
The willingness to pay $v_n(t)$ will depend on the power that consumer $n$   acquired in slots $1, \cdots, t-1$.  All consumers have the same utility function $U(h)$.  If consumer $n$ had  acquired  $x$ kW-slots (out of a total of $t-1$), her willingness to pay would equal  the additional utility she will gain,
\begin{equation} \label{a3}
v_n(t) = U(x+1) - U(x).
\end{equation}
Thus the consumer is myopic: her willingness to pay is unaffected by her opportunities to make future purchases in slots $t+1, \cdots, T$.  The demand function is obtained from \eqref{a2} and \eqref{a3}.  Note that although consumers are myopic, their purchasing decisions depend on  previous decisions. Let $x_i, i=0, \cdots, t-1$, be the number of consumers that have purchased $i$ kW-slots during the first $(t-1)$ spot markets.

Consider the convex case: $U(h)-U(h-1)$ is non-decreasing.  Here, the demand function is

\begin{figure*}[ht]

\begin{equation} \label{a4}
q_t(\pi) = \left \{
\begin{array}{ll}
0 &\mbox{ if } \pi > U(t) - U(t-1) \\
x_{t-1} & \mbox { if }  U(t) - U(t-1) \ge \pi > U(t-1) - U(t-2) \\
x_{t-1}+x_{t-2} & \mbox { if }  U(t-1) - U(t-2) \ge \pi > U(t-2) - U(t-3) \\
& \cdots \\
x_{t-1}+\cdots+ x_1 & \mbox{ if } U(2)-U(1) \ge \pi > U(1) - U(0) \\
x_{t-1} + \cdots +x_0 = N & \mbox{ if } U(1) \ge \pi
\end{array}
\right . .
\end{equation} 
\end{figure*}


Now consider the concave case: $U(h)-U(h-1)$ is non-increasing.  Then the demand function is

\begin{figure*}[ht]
\begin{equation} \label{a5}
q_t(\pi) = \left \{
\begin{array}{ll}
0 &\mbox{ if } \pi > U(1) - U(0) \\
x_0 & \mbox { if }  U(1) - U(0) \ge \pi > U(2) - U(1) \\
x_0+x_1 & \mbox { if }  U(2)-U(1) \ge \pi > U(3) - U(2) \\
& \cdots \\
x_0+\cdots+ x_{t-2} & \mbox{ if } U(t-1) - U(t-2) \ge \pi > U(t-2) - U(t-3) \\
x_0 + \cdots +x_{t-1} = N & \mbox{ if } U(t) -U(t-1)\ge \pi 
\end{array}
\right . .
\end{equation} 
\end{figure*}



\begin{figure*}[ht]
\centering
\includegraphics[width=6in]{spot3new.pdf}
\caption{Demand and supply functions for spot market: convex utility (left), concave utility (right).}
\label{fig-spot}
\end{figure*}
Figure \ref{fig-spot} shows the supply and demand functions  for the convex case (left) and the concave case (right).

\begin{figure*}[ht]
\begin{theorem}[Real-time market]
\label{thm:rt-market} 
\balphlist
\item Suppose $U(h) - U(h-1)$ is a non-negative, non-decreasing function of $h$ (with $U(0)=0$). 
Then, the spot price at $t$ is
\begin{equation}
\pi_t =\left \{
\begin{array}{ll}  \min(c^{rt},U(t)-U(t-1)) &\mbox{ if $r_t < x_{t-1}$}\\
                                    \min(c^{rt},U(t-1) -U(t-2)) & \mbox{ if $x_{t-1} \leq r_t < x_{t-1} + x_{t-2} $}\\
                                      \min(c^{rt},U(t-2) -U(t-3)) & \mbox{ if $x_{t-1}+x_{t-2} \leq r_t < x_{t-1} + x_{t-2} +x_{t-3}$}\\
                                       \cdots\\
                                       \min(c^{rt},U(1)) & \mbox{ if $x_{t-1}+x_{t-2}+\ldots + x_1 \leq r_t < N$}\\
                                       0 & \mbox{ if $N \leq r_t$}
                                        \end{array}
                                       \right. \label{a6}
\end{equation}
%The allocation may not be efficient.  

\item Suppose $U(h)- U(h-1)$ is a non-negative, non-increasing function of $h$ (with $U(0)=0$).
Then the spot price at $t$ is
\begin{equation} \label{a7}
\pi_t = \left \{
\begin{array}{ll}
\min(c^{rt}, U(1)-U(0)) & \mbox{ if } r_t < x_0 \\
\min(c^{rt}, U(2)-U(1))& \mbox{ if } x_0 \le r_t< x_0 +x_1  \\
& \cdots \\
\min(c^{rt},U(t)-U(t-1)) & \mbox{ if }  x_0 + \cdots + x_{t-2}   \le        r_t< x_0 + \cdots + x_{t-1} = N \\
0 & \mbox { if } N \leq r_t
\end{array}
\right . .
\end{equation}
%If such a value does not exist, take $k^*=0$. Then, the price in the first $k^*$ spot markets is $c$. After that, the price is $U(k^*+1)-U(k^*)$. 
%The allocation may not be welfare maximizing.
%\end{enumerate}
\end{list}
\end{theorem}
\end{figure*}
\proof{Proof}
From the intersection of the demand and supply functions in Figure \ref{fig-spot} one can read off the 
formulas \eqref{a6} and \eqref{a7} for the spot price.
\endproof
\begin{example}{\rm   An example shows that the allocation achieved by the real time spot market may not be efficient. In order to compare with the forward market for duration differentiated services, let $c^{da} =c^{rt} = C$. Consider one consumer and two periods, $t=1,2$, the supplier's free power is $r_1 = 0, r_2 = 1$.  For the convex utility case take $U(0) = U(1) = 0, U(2) = 10, C=8$.  In slot 1, since $C > U(1)$, $\pi_1 = U(1)$, the consumer will demand 0 power.
In slot 2, the price will be $\pi_2 = U(1) =0$, the consumer's net benefit will be 0, the producer will receive $\pi_2 = 0$. In the duration-differentiated market  (Theorem \ref{thm:market}), at
the competitive allocation the consumer gets 1 kW for 2 slots and pays $U(2) = 10$ (so her net benefit is 0), the producer will purchase 1 kW in the first slot and pay $C=8$, and will use the free power $p_1$  in the second slot and get a net revenue of $U(2) - 8 = 2$.

For the concave utility case take $U(0)=0, U(1) = U(2) = 5$, $C = 2$.  Since $U(1) > C$, the producer will supply 1 kW in slot 1 at price $\pi_1 = C=2$.
In slot 2, the consumer is indifferent between 1 kW and 0 kW.  She may or not consume $p_2 = 1$ at price $\pi_2 = 0$.
So the consumer's net benefit will be $U(1) - C = 3$, the producer's net profit is 0.  In the duration-differentiated competitive allocation, the consumer will only
purchase 1 kW in slot 2 at price 0, resulting in her net utility of 5, the producer's net profit will again be zero.}
\end{example}

\begin{remark}{\rm  Because of the inter-temporal nature of a consumer's utility, her demand in slot $t$ is contingent on her consumption in other slots.  This contingent demand cannot be met by the system of spot  markets, which is therefore not complete.  This system of markets can be completed through forward markets, like the duration-differentiated market.}
\end{remark}

%\subsection{Supply Uncertainty and the Two-stage Market Problem}




==> 04conclusions.tex <==
\section{Conclusions and Future Work} \label{sec-conclusions}



Flexible loads play a critical role in enabling deep renewable integration. 
They enable demand shaping to balance supply variability, and thus offer an effective alternative to 
conventional generation reserves. In this paper, we study a stylized model of flexible loads. These loads are modeled
as requiring constant power level for a specified duration within a delivery window. The flexibility resides in the fact that the power delivery may occur at any subset of the total period. 
%Mathematical problems in the realm of the scheduling and control of these loads were presented. 
%As a result, many supply profiles can service these loads. 

We consider the supplier's decision problems for serving a given set of duration differentiated loads.  We offered a complete characterization of supply adequacy,
an algorithm for allocating supply to meet the loads and the optimal policies for making day-ahead and real-time power purchase decisions. 
We also study a simplified model of a forward market for these duration differentiated loads where supply uncertainty is not explicitly taken into account.  For this market model, we present the centralized solution that maximizes social welfare and characterize an efficient competitive equilibrium. We also contrast this equilibrium with the outcome of a stylized real-time market.
%We then contrast the outcomes in the forward market with those from a stylized real-time market for these loads. Our study suggests possible inefficiencies of the real-time market implementation. 

The theoretical analysis of this work can facilitate further studies required for exploiting load flexibility. For example,  the results of this paper can be used to evaluate the value of flexibility in reducing supplier's cost under different forecast models of renewable generation. Further, since supply adequacy is not assessed at each time instant, forecasting the exact profile of renewable generation may not be necessary.  Instead, the results of this paper suggest that for providing duration-differentiated services, the key metric to be estimated is the supply-duration vector of the renewable generation.
%The supplier's decisions about purchasing power are made based on its estimation of inadequacy of uncertain renewable supply

A natural extension of this work is to incorporate supply uncertainty into the forward market for duration-differentiated services.  In particular, the supplier should take into account the expected cost of its  real-time power purchases while making its decisions in the forward market.  In this setting, the supplier's cost function  should be given by $J(\cdot)$ defined in \eqref{eq:expected_cost2}.  The existence and efficiency of  competitive equilibria with this new cost function remains to be ascertained. Further research with heterogeneous consumers that have different utilities and power requirements is needed. 


%The results in this paper can be expanded in In particular, the study of flexible loads with different power levels, the consideration of heterogeneous suppliers and consumers and the market operation in the presence of supply uncertainty are important directions for future work. 
%FORMULATE THE TWO STAGE MARKET PROBLEM>>>>>
%The demand side approach to power balance requires the utilization of load flexibility to shape demand in response to supply variations. Demand shaping through real-time price signal needs constant price monitoring and instantaneous responses by consumers. Alternatively, consumers can purchase flexible energy services in a forward market and allow the supplier to manage the loads in response to supply variations.  
%We considered one such scenario with flexible loads that require a constant power level to be delivered for certain number of time slots. We addressed the mathematical problems related to scheduling/control and economics for such loads. We characterized supply adequacy and provided an allocation algorithm for distributing available power among consumers. We considered the problem of purchasing supplemental power in case of inadequate supply. We also considered the general case where loads can absorb power at a variable rate. We considered a forward market where consumers can purchase duration-differentiated energy services and showed that there is an efficient competitive equilibrium. We  pointed out the possible inefficiency of a real-time market for flexible loads.
%

